Higgs and the electroweak precision observables in the MRSSM

We briefly review recent progress in the analysis of the Higgs sector of the Minimal R-symmetric Supersymmetric Standard Model. Importance of the interplay between W and Higgs boson masses in constraining the parameter space of the model is shown.

==> TeX/section4.tex <==
\section{Future prospects: Dirac dark matter and collider study}

Up to now we only discussed scenarios in which the lightest Higgs boson is the one observed by the LHC.
Another intriguing possibility is that it is actually a next-to-lightest one, with a lightest one being mainly a $SU(2)_L$ singlet, yet to be detected.
The mass of the SM-like one is then pushed up due to the mixing with the singlet, reducing the need for large radiative corrections.\footnote{This mechanism was already used, in the context of NMSSM, in \cite{Badziak:2013bda}.}
Current LHC data still allow for substantial, roughly less than 10\%, admixture of singlet component in the 125 GeV state \cite{LHC_Higgs_ATLAS,Khachatryan:2014jba}.

Since the mass of the $\phi_S$ state is controlled both by $m_S$ and $M_B^D$ (where the latter one enters into the Higgs mass matrix through D-term contribution), 
\begin{equation}
m_{\phi_S \phi_S}^2 =  m_S^2 + 4 (M_B^D)^2+\frac{\lambda_d^2 v_d^2+\lambda_u^2 v_u^2}{2},
\end{equation}
both of these parameters must be small, below 100 GeV. 
This leads to light bino/singlino Dirac neutralinos, which in our study are most of the time lighter than 30 GeV.\footnote{This limit comes from the Higgs sector of the model.}
It is than important to check if such a light particle is not excluded by current LHC data.
Figure \ref{fig:exclusion_limit} shows (in blue) parameter region allowed by constrains coming from chargino and neutralino production at the LHC, namely $pp \to \tilde{\chi}_i^0 \tilde{\chi}_j^0, \tilde{\chi}_i^0 \tilde{\chi}_j^\pm, \tilde \chi_i^0 \tilde{\rho}_j^\pm$, for parameters defined in  tab. \ref{tab:BMP}. 
Indexes $i,j$ run from 1 to 4 in case of neutralinos $\tilde{\chi}^0$ and to 2 in case of charginos $\tilde{\chi}^\pm, \tilde{\rho}^\pm$.
LO predictions were generated with \texttt{Herwig++} using \texttt{SARAH} generated UFO model \cite{Degrande:2011ua,Staub:2012pb} and checked against experimental results from refs. \cite{Aad:2014nua,Aad:2014vma,TheATLAScollaboration:2013hha} using \texttt{CheckMate}~\cite{Drees:2013wra}.

\begin{table}[t]
\begin{center}
%\begin{tabular}{l|r}
%%\toprule
%&BMP4\\
%\hline
%$\tan\beta$  & 40\\
%%$B_\mu$      & $200^2$\\
%$\lambda_d$, $\lambda_u$&   $0,0$ \\
%$\Lambda_d$, $\Lambda_u$&  $0,-1.1$\\
%%$m_S^2$ & $80^2$\\
%%$m_{R_u}^2$ & $1000^2$\\
%%$M_O^D$& $1500$\\
%%$m_T^2$, $m_O^2$&$3000^2,1000^2$\\
%$m_{Q;1,2}^2$, $m_{Q;3}^2$&$2500^2,700^2$\\
%$m_{D;1,2}^2$, $m_{D;3}^2$&$2500^2,1000^2$\\
%$m_{U;1,2}^2$, $m_{U;3}^2$&$2500^2,700^2$\\
%%$m_{L;1,2}^2$, $m_{E;1,2}^2$&$1000^2$\\
%%$m_{L;3,3}^2$, $m_{E;3,3}^2$ & $500^2$, $\sim 100^2$\\
%%$m_{R_d}^2$&$700^2$\\
%%\bottomrule
%\end{tabular}
\begin{tabular}{ccccccc}
  $\tan\beta$ & $\lambda_d = \lambda_u$ & $\Lambda_d$ & $\Lambda_u$ & $m_{Q;1,2}^2 = m_{D;1,2}^2 = m_{U;1,2}^2$ & $m_{Q;3}^2 = m_{U;3}^2$ & $m_{D;3}^2$\\
  \midrule
  40 & 0 & 0 & -1.1 & $2500^2$ & $700^2$ & $1000^2$
\end{tabular}
\end{center}
\caption{Benchmark point for the following plots. Dimensionful parameters are given in
GeV or GeV${}^2$, as appropriate.}
\label{tab:BMP}
\end{table}
\begin{figure}
  \centering
  \includegraphics[width=0.6\textwidth]{img/LHC_bounds.pdf}
  \caption{Region excluded by direct search of chargino and neutralino production, as given by \texttt{CheckMate}~\cite{Drees:2013wra}.
      Experimental data come from refs. \cite{Aad:2014nua,Aad:2014vma,TheATLAScollaboration:2013hha}.
  }
  \label{fig:exclusion_limit}
\end{figure}

Since for a bino/singlino dark matter we need to rely on stau coanihilation to get the DM relic abundance lower than the limit set by Planck+WP+highL+BAO \cite{Ade:2013zuv}.
This implies the existence of staus with mass of around 150 GeV.
The final question, which is still under investigation, is whether all those requirements can be agreed with data coming from direct detection experiments, mainly from the LUX experiment \cite{Akerib:2012ys}.
Preliminary analysis suggests that it will give non trivial constraints on parameter space.

\FloatBarrier

==> TeX/section45.tex <==
\section{Higher order corrections to Higgs mass}

\begin{figure}[ht]
\centering
  \includegraphics{img/2L_sgluon_correction}
  \includegraphics{img/2L_gluino_correction}
  \caption{Two-loop diagrams contributing  to the Higgs boson that depend on the Dirac mass $M_O^D$ and the
    soft sgluon mass $m_O$. Only diagrams involving tops/stops are draw.}
  \label{fig:2l_diagrams}
\end{figure}

\begin{figure}[th]
\centering
\includegraphics[width=0.4\textwidth]{img/higgs_color_contrb.pdf}
\caption{
Decomposition of two-loop contributions given for $m_O=2$~TeV.
Remaining parameters are fixed to BMP3 from \cite{Diessner:2015yna}.
}
\label{img:mgmocontrb}
\end{figure}

Beyond the one-loop level Higgs mass starts to be sensitive to pure-QCD sector of the model.
Of most interest are the corrections coming from exchange of sgluons and Dirac gluinos, which are a novel feature of the MRSSM (compared to MSSM).
Figure \ref{fig:2l_diagrams} shows most relevant contributions to the two-loop effective potential depending on Dirac gluino mass $M_O^D$ and sgluon soft-mass parameter $m_O$.
As was shown in \cite{Diessner:2015yna}, the two-loop dependence on $M_O^D$ can be decomposed into leading part coming from sgluon exchange followed by sublideaing one from gluino exchange.
The sgluons contribution is always positive and larger than the one coming from gluino, which turn negative for large values of $M_O^D$.
Still the main correction comes from MSSM-like diagrams with gluon exchange, accounting for bulk of the +4--5 GeV contribution.
This allowed to reduce a minor tension present in \cite{Diessner:2014ksa} between Higgs and W boson masses.
\FloatBarrier
